Exploring Perceptual Limitation of Multimodal Large Language Models

Multimodal Large Language Models (MLLMs) have recently shown remarkable perceptual capability in answering visual questions, however, little is known about the limits of their perception. In particular, while prior works have provided anecdotal evidence of MLLMs' sensitivity to object size, this phenomenon and its underlying causes have not been explored comprehensively. In this work, we quantitatively study the perception of small visual objects in several state-of-the-art MLLMs and reveal a pervasive limitation in answering questions about small objects in images. Next, we identify four independent factors that can contribute to this limitation -- object quality, size, distractors, and location -- and conduct controlled intervention studies to measure the effect of each factor on MLLMs' perception. In particular, we find that lower object quality and smaller object size can both independently reduce MLLMs' ability to answer visual questions. More surprisingly, we find that the location of the object in the image and the presence of visual distractors can also significantly reduce MLLMs' question answering accuracy. Our study provides a better understanding of the perceptual limitation of MLLMs and contributes new evaluation protocols for analyzing the perception of future MLLMs. To facilitate further investigations, we release our code and data.

==> figs/fig_distractor_illstration.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[trim=0 0 0 0, clip, width=0.95\textwidth]{figs/distractor_illstration.pdf}
  \vspace{-0.5cm}
  \caption{
  An illustrative example of the dataset constructed to vary the number of distractors. We show the texts with font size of 3.
  }
  \label{fig:cut_example}
  \vspace{-0.1cm}
\end{figure*}

==> sections/discussion.tex <==
\section{Discussion}

\begin{table}[h!]
\centering
\small
\caption{Intervals of number of pixel values (\textbf{\# Pixels}) within the bounding box after the input images are unified to size \textbf{224$\times$224} on 5 data quantiles of GQA and TextVQA tested in~\cref{sec:motivation}, and the average number of object/textual distractors (\textbf{\# D}) in two datasets. \\}
\begin{tabular}{c|l|l|l|l}
\toprule
\textbf{Data} & \multicolumn{2}{c|}{\textbf{GQA}} & \multicolumn{2}{c}{\textbf{TextVQA}} \\
\textbf{Quantile} & \# Pixels & \# D & \# Pixels & \# D \\
\midrule
1 & [100, 1409]   & 19.2 & [26, 80]    & 14.9 \\
2 & [1409, 5043]  & 18.1 & [80, 143]   & 13.8 \\
3 & [5045, 11967] & 17.4 & [143, 296]  & 13.1 \\
4 & [11971, 24571]& 16.7 & [296, 697]  & 11.7 \\
5 & [24588, 50176]& 14.6 & [698, 50176]& 7.6 \\
\bottomrule
\end{tabular}
\label{tab:ranges}
\end{table}



\textbf{What is the contribution of each factor on the low performance of smaller objects?}
To better understand to what extent each factor affects the performance in~\autoref{fig:motivation}, we compute the range of the number of pixels within each quantile after the input images are unified to 224$\times$244. For models with higher resolutions, the number of pixels of the input images increases proportionally. We also compute the average number of textual distractors by the number of OCR tokens in each quantile of TextVQA. The statistics are presented in~\autoref{tab:ranges}.

In TextVQA, the resolution of the first three quantiles is notably limited. The dataset has an average text length of 8.77 characters. Considering that a text string comprising nine characters approximately covers 200 pixels under a sampling rate of 8, a large portion of images within the first three quantiles of the TextVQA fall below the observed sampling rate threshold, which provides evidence for their low performance. However, the impact of object quality is much less significant when it reaches a threshold (\autoref{fig:quality}), suggesting that the increased accuracy of the rest of TextVQA and nearly the entire GQA cannot be attributed to improvements in image quality. In addition, ~\autoref{fig:distract} indicates that the effects of distractors are most significant when the number increases to five and the trend is gradually stabilized beyond this point. This might suggest that distractor numbers are not the main cause of the overall trend and that object size plays a more critical role in it. We report on further analysis in the Appendix.


\textbf{What is causing the variance in positional bias?}
The different positional bias observed from~\cref{sec:location} may stem from the bias from textual training data, predominantly from left to right and at the image centers, potentially under-representing text on the right side and the margin of images. 
However, the notable performance decline observed in the first row of Fuyu-8B does not correspond to this data set bias hypothesis. We assume that this unique performance disparity in Fuyu-8B may be attributable to its singular decoder-based transformer architecture. We will explore this phenomenon further in the Appendix.
